3D surface profilometry using neutral helium atoms

Three-dimensional mapping of surface structures is important in a wide range of biological, technological, healthcare and research applications, including taxonomy, microfluidics and fabrication. Neutral helium atom beams have been established as a sensitive probe of topography and have already enabled structural information to be obtained from delicate samples, where conventional probes would cause damage. Here, we demonstrate empirical reconstruction of a complete surface profile using measurements from a scanning helium microscope (SHeM), using the heliometric stereo method and a single detector instrument geometry. Results for the surface profile of tetrahedral aluminum potassium sulphate crystals demonstrate the areas of surfaces and facet orientations can be recovered to within 5% of the expected values.

==> gfx/new_pinhole_plate_1.tex <==
%% Creator: Inkscape 1.2.2 (732a01da63, 2022-12-09), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'new_pinhole_plate.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{246bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,1.46747967)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0.41195328,1.08230548){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\theta$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{new_pinhole_plate.pdf}}%
    \put(0.6096515,1.2385161){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Original pinhole plate\end{tabular}}}}%
    \put(0.40604574,1.43374516){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Incident He beam\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{new_pinhole_plate.pdf}}%
    \put(0.494,0.81849369){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$xy$ Scanning plane\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{new_pinhole_plate.pdf}}%
    \put(0.14578367,1.09389274){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}Rotation axis\end{tabular}}}}%
    \put(0.26977538,1.29296496){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}Pinhole\end{tabular}}}}%
    \put(0.00376485,1.43462784){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\textrm{(a)}\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{new_pinhole_plate.pdf}}%
    \put(0.505,0.68683041){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}New pinhole plate\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=5]{new_pinhole_plate.pdf}}%
    \put(0.40439425,0.10571908){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}Sample\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=6]{new_pinhole_plate.pdf}}%
    \put(0.49077848,0.02246095){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$xy$ Scanning plane\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=7]{new_pinhole_plate.pdf}}%
    \put(0.10732042,0.05614961){\color[rgb]{0,0,0}\makebox(0,0)[t]{\lineheight{1.25}\smash{\begin{tabular}[t]{c}Rotation axis\end{tabular}}}}%
    \put(0.13828663,0.61290488){\color[rgb]{0,0,0}\makebox(0,0)[t]{\smash{\begin{tabular}[t]{c}Sample position \\rotated relative \\to beam\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=8]{new_pinhole_plate.pdf}}%
    \put(0.0037649,0.78102292){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\textrm{(b)}\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=9]{new_pinhole_plate.pdf}}%
    \put(0.405,0.220304){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\ang{35}$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=10]{new_pinhole_plate.pdf}}%
    \put(0.85364169,1.10069152){\color[rgb]{0,0,0}\makebox(0,0)[t]{\smash{\begin{tabular}[t]{c}To detector\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=11]{new_pinhole_plate.pdf}}%
    \put(0.72467699,0.58114142){\color[rgb]{0,0,0}\makebox(0,0)[t]{\smash{\begin{tabular}[t]{c}To detector\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=12]{new_pinhole_plate.pdf}}%
  \end{picture}%
\endgroup%

